Visual Analysis of Prediction Uncertainty in Neural Networks for Deep Image Synthesis

Ubiquitous applications of Deep neural networks (DNNs) in different artificial intelligence systems have led to their adoption in solving challenging visualization problems in recent years. While sophisticated DNNs offer an impressive generalization, it is imperative to comprehend the quality, confidence, robustness, and uncertainty associated with their prediction. A thorough understanding of these quantities produces actionable insights that help application scientists make informed decisions. Unfortunately, the intrinsic design principles of the DNNs cannot beget prediction uncertainty, necessitating separate formulations for robust uncertainty-aware models for diverse visualization applications. To that end, this contribution demonstrates how the prediction uncertainty and sensitivity of DNNs can be estimated efficiently using various methods and then interactively compared and contrasted for deep image synthesis tasks. Our inspection suggests that uncertainty-aware deep visualization models generate illustrations of informative and superior quality and diversity. Furthermore, prediction uncertainty improves the robustness and interpretability of deep visualization models, making them practical and convenient for various scientific domains that thrive on visual analyses.

==> sections/bayesian-methods.tex <==
\textbf{Bayesian Methods.} Probabilistic Bayesian methods enforce flexible prior distributions on the parameters of DNN to facilitate appropriate regularization and precise estimation of the predictive uncertainty~\cite{blck15, deep.ensembles}. Unfortunately, many of these methods incur prohibitively expensive computation costs for state-of-the-art DNNs that often contain millions of parameters. In literature, techniques such as Laplace approximation \cite{mack92}, stochastic gradient MCMC \cite{mafb17}, and variational inference \cite{hahn19} are significantly slower compared to many of the first-order \cite{kiba14} and second-order methods \cite{xuez21} used in training DNNs. More importantly, the effects of batch size, batch/layer normalization \cite{bakh16}, dropout \cite{srhk14, gagh16}, and adversarial weight perturbation \cite{limc22} are much better understood in the context of many of the first and second order methods. State-of-the-art language \cite{decl18} and vision models \cite{bicx20} and recommender systems \cite{nams19} show a notable boost in performance when these effects are scrupulously moderated.

%% re-introducing some of the references here without which the argument would not stand strong
%% Bayesian methods are always better suited for providing uncertainties in a principled way; however, their applications pose certain practical challenges; some of these challenges are related to computation, but the others are related to the fact that no one knows very accurately yet how to tune some of the training configs to achieve the SOTA results with Bayesian methods

%%*** I am cutting down some texts as this seems too much in the context of this paper. ***%%

% \textbf{Bayesian Methods.} Probabilistic Bayesian methods enforce flexible prior distributions on the parameters of DNN to facilitate appropriate regularization and precise estimation of the predictive uncertainty~\cite{blck15, lapb17}. Unfortunately, many of these methods incur prohibitively expensive computation costs for state-of-the-art DNNs that often contain millions of parameters. In general, techniques such as Laplace approximation \cite{mack92,lehf20}, stochastic gradient MCMC \cite{mafb17, macf15}, and variational inference \cite{hahn19, yizh18, rekv21} are significantly slower compared to many of the first-order \cite{kiba14, xiss21, wuws22} and second-order methods \cite{xuez21, angk20} used in training DNNs. More importantly, the effects of batch size \cite{yolr19}, batch/layer normalization \cite{bakh16}, dropout \cite{srhk14, gagh16}, learning-rate schedule \cite{yojc19}, label smoothing \cite{mukh19}, and adversarial weight perturbation \cite{zhgy22, bamt21, limc22} are much better understood in the context of many of the first and second order methods. State-of-the-art language \cite{decl18, yolr19} and vision models \cite{bicx20, chhg21} and recommender systems \cite{nams19} show a notable boost in performance when these effects are scrupulously moderated.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Probabilistic methods enforce flexible prior distributions on the parameters of DNN to facilitate appropriate regularization and precise estimation of the predictive uncertainty  \cite{blck15, lapb17}. Unfortunately, many of these methods incur prohibitively expensive computation costs for state-of-the-art DNNs that often contain millions of parameters. In general, techniques such as Laplace approximation \cite{mack92, saki16, lehf20, ribb18}, stochastic gradient MCMC \cite{mafb17, macf15, wete11}, and (online) variational inference \cite{wapb11, beal2003, likh18, meng17, hahn19, hobl15, yizh18, rekv21} are significantly slower compared to many of the first-order \cite{smdb20, kiba14, xiss21, wuws22, saqu18, hawl21, xiss21, sumd13} and second-order methods \cite{xuez21, angk20} used in training DNNs. More importantly, the effects of batch size \cite{yojc19, yolr19}, batch/layer normalization \cite{iosz15, bakh16}, Dropout \cite{srhk14, gagh16}, learning-rate schedule \cite{yojc19}, label smoothing \cite{mukh19}, and adversarial weight perturbation \cite{anfl22, fokm20, duzf22, zhgy22, bamt21, limc22} are much better understood in the context of many of the first and second order methods. State-of-the-art language \cite{vasp17, liog19, decl18, yolr19} and vision models \cite{bicx20, chhg21, hezr16, zako16, ruds15} and recommender systems \cite{nams19} show a notable boost in performance when these effects are scrupulously moderated.


==> sections/deterministic-methods.tex <==
% \subsubsection{Deterministic Methods}

\textbf{Deterministic Methods.} Enabling deterministic models with prediction uncertainty is counter-intuitive. In the absence of any principled approach to introduce such diversity, one resorts to two broad classes of techniques. In one approach, a single network is explicitly modelled and trained to quantify uncertainties \cite{evidential.neural.networks, prior.network}. Many works along this thread model a distribution over the target distribution to quantify the uncertainty. The other methods use additional components, extrinsic to the prediction models, to produce uncertainty estimates \cite{second.opinion.medical,density.estimation.in.representation.space}.

%Evidential neural networks \cite{evidential.neural.networks} also optimize the parameterization of a single Dirichlet network. The loss formulation is derived by using subjective logic and interpret the logits as multinomial opinions or beliefs, as introduced in Evidence or Dempster-Shafer theory \cite{dempster1968generalization}. Evidential neural networks set the total amount of evidence in relation with the number of classes and conclude a value of uncertainty from this, i.e. receiving an additional "I don't know class". The loss is formulated as expected value of a basic loss, as for example categorical cross entropy, with respect to a Dirichlet distribution parameterized by the logits. Additionally, a regularization term is added, encouraging the network to not consider features that provide evidence for multiple classes at the same time, as for example a circle is for 6 and 8. Due to this, the networks do not differentiate between data uncertainty and model uncertainty, but learn whether they can give a certain prediction or not.  \cite{regularized.evidential.networks} extended this idea by differentiating between acuity and dissonance in the collected evidence in order to better separate in- and out-of-distribution samples. For that, two explicit data sets containing overlapping classes and out-of-distribution samples are needed to learn a regularization term. Amini et al. \cite{alex2019} transferred the idea of evidential neural networks from classification tasks to regression tasks by learning the parameters of an evidential normal inverse gamma distribution over an underlying Normal distribution. Charpentier et al. \cite{charpentier2020posterior} avoided the need of OOD data for the training process by using normalizing flows to learn a distribution over a latent space for each class. A new input sample is projected onto this latent space and a Dirichlet distribution is parameterized based on the class wise densities of the received latent point. 

%Beside the Dirichlet distribution based approaches described above, several other internal approaches exist. In \cite{liang2017enhancing}, a relatively simple approach based on small pertubations on the training input data and the temperature scaling calibration is presented leading to an efficient differentiation of in- and out-of-distritbuion samples. Mo$\dot{\text{z}}$ejko et al. \cite{inhibited.softmax} made use of the inhibited softmax function. It contains an artificial and constant logit that makes the absolute magnitude of the single logits more determining in the softmax output. Van Amersfoort et al. \cite{kernel.network} showed that Radial Basis Function (RBF) networks can be used to achieve competitive results in accuracy and very good results regarding uncertainty estimation. RBF networks learn a linear transformation on the logits and classify inputs based on the distance between the transformed logits and the learned class centroids. In \cite{kernel.network}, a scaled exponentiated $L_2$ distance was used. The data uncertainty can be directly derived from the distances between the centroids. By including penalties on the Jacobian matrix in the loss function, the network was trained to be more sensitive to changes in the input space. As a result, the method reached good performance on out-of-distribution detection. In several tests, the approach was compared to a five members deep ensemble \cite{deep.ensembles} and it was shown that this single network approach performs at least equivalently well on detecting out-of-distribution samples and improves the true-positive rate. \\

%For regression tasks, Oala et al. \cite{interval.neural.networks.uncertainty.score} introduced an uncertainty score based on the lower and an upper bound output of an interval neural network. The interval neural network has the same structure as the underlying deterministic neural network and is initialized with the deterministic network's weights. In contrast to Gaussian representations of uncertainty given by a standard deviation, this approach can give non-symmetric values of uncertainty. Furthermore, the approach is found to be more robust in the presence of noise. Tagasovska and Lopez-Paz \cite{tagasovska2019single} presented an approach to estimate data and model uncertainty. A simultaneous quantile regression loss function was introduced in order to generate well-calibrated prediction intervals for the data uncertainty.  The model uncertainty is quantified based on a mapping from the training data to zero, based on so called Orthonormal Certificates. The aim was that out-of-distribution samples, where the model is uncertain, are mapped to a non-zero value and thus can be recognized. Kawashima et al. \cite{kawashima2020aleatoric} introduced a method which computes virtual residuals in the training samples of a regression task based on a cross-validation like pre-training step. With original training data expanded by the information of these residuals, the actual predictor is trained to give a prediction and a value of certainty. The experiments indicated that the virtual residuals represent a promising tool in order to avoid overconfident network predictions. 

==> sections/test-time-augmentation.tex <==
\textbf{Test-time Augmentation Methods.} The test-time augmentation methods derive inspiration from the utility of ensemble methods and enrich model training using adversarial examples \cite{Ayhan.2018}. In applications such as medical imaging \cite{wang2019aleatoric}, procuring labelled data is challenging, so one has to resort to data augmentation techniques to circumvent problems related to data scarcity during training. Interestingly, the same augmentation techniques can be applied to the test data. The augmented data provide a complementary view of the original test data; hence, a user can be better poised to infer the test-time uncertainty~\cite{shanmugam2020and, molchanov2020greedy}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The test-time augmentation methods derive inspiration from the utility of ensemble methods and enrichment of model training using adversarial examples \cite{Ayhan.2018}. In applications such as medical imaging \cite{wang2018automatic,wang2019aleatoric,Ayhan.2018,moshkov2020test}, procuring labelled data is challenging, so one has to resort to data augmentation techniques to circumvent problems related to data paucity during training. Interestingly, the same augmentation techniques can be applied to the test data. The augmented data provide a complementary view of the original test data; hence, a user can be better poised to infer the test-time uncertainty. 

% Such techniques seem appealing and convenient as they do not require practitioners to change the model training or collect more data. However, the augmentation needs to be carefully balanced not to generate samples beyond the distribution seen during the training time. Nevertheless, when done appropriately, test-time augmentation can rectify many predictions and provide an accurate estimate of the uncertainty. One can further propose creative strategies for learning the mapping from a subset of the augmented test samples to generate more precise predictions and cater to different facets of uncertainty \cite{shanmugam2020and, molchanov2020greedy, kim2020learning}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Inspired by ensemble methods and adversarial examples \cite{Ayhan.2018}, the test time data augmentation is one of the simpler predictive uncertainty estimation techniques. The basic method is to create multiple test samples from each test sample by applying data augmentation techniques on it and then test all those samples to compute a predictive distribution in order to measure uncertainty. The idea behind this method is that the augmented test samples allow the exploration of different views and is therefore capable of capturing the uncertainty. Mostly, this technique of test time data augmentations has been used in medical image processing \cite{wang2018automatic,wang2019aleatoric,Ayhan.2018,moshkov2020test}. One of the reasons for this is that the field of medical image processing already makes heavy use of data augmentations while using deep learning \cite{ronneberger2015u}, so it is quite easy to just apply those same augmentations during test time to calculate the uncertainties. Another reason is that collecting medical images is costly, thus forcing practitioners to rely on data augmentation techniques. 
%Moshkov et al. \cite{moshkov2020test} used the test time augmentation technique for cell segmentation tasks. For that, they created multiple variations of the test data before feeding it to a trained UNet or Mask R-CNN architecture. Following, they used a majority voting to create the final output segmentation mask and discuss the policies of applying different augmentation techniques and how they affect the final predictive results of the deep networks.

%Overall, test time augmentation is an easy method for estimating uncertainties because it keeps the underlying model unchanged, requires no additional data, and is simple to put into practice with off-the-shelf libraries. Nonetheless, it needs to be kept in mind that during applying this technique, one should only apply valid augmentations to the data, meaning that the augmentations should not generate data from outside the target distribution. According to \cite{shanmugam2020and}, test time augmentation can change many correct predictions into incorrect predictions (and vice versa) due to many factors such as the nature of the problem at hand, the size of training data, the deep neural network architecture, and the type of augmentation. To limit the impact of these factors, Shanmugam et al. \cite{shanmugam2020and} proposed a learning-based method for test time augmentation that takes these factors into consideration. In particular, the proposed method learns a function that aggregates the predictions from each augmentation of a test sample. Similar to \cite{shanmugam2020and}, Molchanov et al. \cite{molchanov2020greedy} proposed a method, named “greedy Policy Search”, for constructing a test-time augmentation policy by choosing augmentations to be include in a fixed-length policy. Similarly, Kim et al. \cite{kim2020learning} proposed a method for learning a loss predictor from the training data for instance-aware test-time augmentation selection. The predictor selects test-time augmentations with the lowest predicted loss for a given sample.

%Although learnable test time augmentation techniques \cite{shanmugam2020and, molchanov2020greedy, kim2020learning} help to select valid augmentations, one of the major open question is to find out the effect on uncertainty due to different kinds of augmentations. It can for example happen that a simple augmentation like reflection is not able to capture much of the uncertainty while some domain specialized stretching and shearing captures more uncertainty. It is also important to find out how many augmentations are needed to correctly quantify uncertainties in a given task. This is particularly important in applications like earth observation, where inference might be needed on global scale with limited resources.

==> sections/uncertainty.tex <==
\section{Uncertainty in Deep Neural Networks}
\label{sec:uncertainty}

The wide popularity of deep learning techniques \cite{lebh15} does not accord with the overarching concern about their interpretability, robustness and generalizability in real-world applications \cite{zhbh16}. In general, the inability of the DNNs to cater to uncertainty estimates and the well-known issues related to their calibration can undermine the superior empirical gains they achieve in applications like natural language processing \cite{vasp17, liog19}, computer vision \cite{bicx20, chhg21, hezr16, zako16},  recommender systems \cite{nams19}, and visual analytics~\cite{va4ml_survey}. Condensing this gap is a daunting  task, as the margin of error in most scientific applications is minimal \cite{zhaj21}. Furthermore, the sources and characterization of uncertainty vary widely from one application domain to the other. Hence, formalizing and generalizing the techniques to measure and quantify the uncertainty in an \textit{application-agnostic} way remains an open challenge. In what follows, we briefly explain some of the  sources of uncertainty in DNNs and different methods adopted to emulate and address the same.

\subsection{Sources of Uncertainty in Applications of DNNs}

The predictive uncertainty \cite{blck15, deep.ensembles} of a DNN can be broadly categorized into two groups -- \emph{data or aleatoric uncertainty} and \emph{model or epistemic uncertainty}. Data uncertainty arises due to errors and noise in measurement systems. For example, in an image classification task, the images collected might be corrupted due to some glitch in the mechanical systems that capture them. Similarly, in a climate prediction problem, the noises due to sensor miscalibration and mechanical stress can contaminate the observed measurements.

The modeling (epistemic) uncertainty, on the other hand, can be due to multiple reasons. First, the state-of-the-art DNN models produce a compact representation of the real-world system that generates the observations. Such parsimony often leads to prediction errors and associated uncertainty. Second, over-parameterized networks often exhibit \emph{double descent} \cite{nakb21} -- a phenomenon that leads to sharper prediction and lower uncertainty. Third, many DNNs must be carefully tuned using drop-connect \cite{wazz13}, dropout \cite{gagh16, hisk12}, learning-rate warm-up and decay \cite{yojc19}, regularization \cite{chsn19} etc. Different decisions for such parameters lead to different learned configurations of the models, which further leads to considerable variability in prediction.

\subsection{Techniques for Modeling Uncertainty in DNNs}
In the following, we first briefly highlight several existing methods of uncertainty modeling in DNNs and then discuss deep ensembles and MC-Dropout-based uncertainty estimation in detail, which are employed in our work to capture prediction uncertainty of image-based deep visualization models.

\input{sections/deterministic-methods}
\input{sections/test-time-augmentation}
\input{sections/bayesian-methods}

\input{sections/ensemble-methods}
\input{sections/dropout}
\input{sections/dropout-dnns}

